Quadratic neural networks for solving inverse problems

In this paper we investigate the solution of inverse problems with neural network ansatz functions with generalized decision functions. The relevant observation for this work is that such functions can approximate typical test cases, such as the Shepp-Logan phantom, better, than standard neural networks. Moreover, we show that the convergence analysis of numerical methods for solving inverse problems with shallow generalized neural network functions leads to more intuitive convergence conditions, than for deep affine linear neural networks.

==> Makefile <==
MAIN = FriSchShi23_preprint3

.PHONY: default full final clean check whoareyou bib help

default:
	pdflatex --file-line-error $(MAIN).tex

full:
	latexmk -pdf --file-line-error $(MAIN).tex

final:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex
	biber --output_format=bibtex --output_resolve $(MAIN) -O biber.bib
	sed $(MAIN).tex -e '/^\\def\\notfinal{}/d' > $(MAIN)_final.tex
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN)_final.tex
	latexmk -c $(MAIN).tex
	latexmk -c $(MAIN)_final.tex

clean:
	latexmk -c $(MAIN).tex
	rm -f $(MAIN).bbl $(MAIN).run.xml $(MAIN).thm $(MAIN).pdf

check:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex

whoareyou:
	@echo $(MAIN)

bib:
	$(eval AUX := $(shell mktemp -d))
	latexmk -gg -pdf -jobname=extract -pdflatex="/usr/bin/pdflatex --file-line-error --shell-escape --synctex=1 %O '\def\extract{}\input{%S}'" -output-directory=${AUX} ${MAIN}.tex
	biber --output_format=bibtex --output_resolve -O ${AUX}/extract.bib ${AUX}/extract
	echo "\n%% Warning: This file is autogenerated, editing might be futile.\n" > csc.bib
	cat ${AUX}/extract.bib >> csc.bib

help:
	@echo ""
	@echo "make targets are:"
	@echo ""
	@echo "  default (default):"
	@echo "    just builds the tex file (without bibliography)"
	@echo ""
	@echo "  bib:"
	@echo "    extracts bibliography to csc.bib"
	@echo ""
	@echo "  full:"
	@echo "    builds the tex file (with bibliography)"
	@echo ""
	@echo "  final:"
	@echo "    extracts the bibliography into a local bib file"
	@echo "    creates an $(MAIN)_final.tex file using the extracted bib data"
	@echo ""
	@echo "  clean:"
	@echo "    cleans up temporary files"
	@echo ""
	@echo "  (check):"
	@echo "    used by the papercheck deamon, same as full but doesn't halt on error"
	@echo ""
	@echo "  (whoareyou):"
	@echo "    used by the papercheck daemon to identify this Makefile"
	@echo ""


